Transformer-based Learned Image Compression for Joint Decoding and Denoising

This work introduces a Transformer-based image compression system. It has the flexibility to switch between the standard image reconstruction and the denoising reconstruction from a single compressed bitstream. Instead of training separate decoders for these tasks, we incorporate two add-on modules to adapt a pre-trained image decoder from performing the standard image reconstruction to joint decoding and denoising. Our scheme adopts a two-pronged approach. It features a latent refinement module to refine the latent representation of a noisy input image for reconstructing a noise-free image. Additionally, it incorporates an instance-specific prompt generator that adapts the decoding process to improve on the latent refinement. Experimental results show that our method achieves a similar level of denoising quality to training a separate decoder for joint decoding and denoising at the expense of only a modest increase in the decoder's model size and computational complexity.

==> Figure/ablation_RD-curve.tex <==
\begin{figure}[t]
\centering
\subfigure[SFT vs. Prompt]{
\centering 
\includegraphics[width=0.46\linewidth]{Figure/RD-curve/ablation_performance(SFT)_v8.png}
}
\hspace{-0.35cm}
\subfigure[Numbers of Prompt]{
\centering
\includegraphics[width=0.46\linewidth]{Figure/RD-curve/different_IPnumber(SFT)_v6.png}
}
\caption{}
\label{fig:ablation}
\vspace{-0.2cm}
\end{figure}

==> Section/2_related.tex <==
\section{Related Work}
\label{sec:related}
